Fluctuations of lattice zonotopes and polygons

Following Barany et al., who proved that large random lattice zonotopes converge to a deterministic shape in any dimension after rescaling, we establish a central limit theorem for finite-dimensional marginals of the boundary of the zonotope. In dimension 2, for large random convex lattice polygons contained in a square, we prove a Donsker-type theorem for the boundary fluctuations, which involves a two-dimensional Brownian bridge and a drift term that we identify as a random cubic curve.

==> Parties/Development/4brownianbridge.tex <==
Covariance of  $n^{- \frac{d+2}{2(d+1)}} \AA_\uu ^n$ :

$$ \Gamma_\uu ^n = \left(\frac{\zeta(d)}{\zeta(d+1)}\right)^{\frac{1}{d+1}} (d+1)! \int_{\mathcal{C}( \aa \leq 1, u \geq 0)} \xx^\intercal \xx d\xx + O\left(n \right) $$


==> Parties/Development/7properties.tex <==
Proof of the theorem. Let $F$ be a bounded, continuous functional on the set
of continuous functions: $[0,1]\to \R$. We may assume that $|F|\leq 1$.

Let
$\varepsilon>0$. First, thanks to Proposition 1, there exists $t>0$ such that
with probability $>1-\varepsilon$, $|n^{-2/3}(X(A_n, S'_n)|<t$
and $|n^{-2/3}(Y(B_n, E'_n)|<t$.

Theorem ?? tells us that $n$ large enough, for all $n_1, n_2$ such that
$|n_1-n|<tn^{2/3}$ and $|n_2-n|<tn^{2/3}$,
$$|E F(f_n|E_n-S_n=(n_1,n_2))- E F(B)|\leq \varepsilon$$
where $B$ is a Brownian bridge.
Let $G_n$ be the event $|X(E_n-S_n)-n|<tn^{2/3}$ and $|Y(E_n-S_n)-n|<tn^{2/3}$
Then for  $n$ large enough, 
$$|E F(f_n{\bf 1}_{G_n})- E F(B)|\leq \varepsilon$$
On the other hand, since $P(G_n^c)<\varepsilon$ and by boundedness of $F$,
$$|E F(f_n{\bf 1}_{G_n^c})- E F(B)|\leq \varepsilon$$
which proves the Theorem.

==> historique/1dec_5polygons.tex <==

Consider a random, uniform lattice convex polygon $P_n$ contained in the
square $[-n,n]^2$. Then a direct consequence of the papers
by Barany, Sinai and Vershik is that $P_n$ converges in distribution to a deterministic
shape which is the union of 4 arcs of parabola.

Let us introduce some notation. Let $A_n=(A'_n, A''_n)$ be the western-most point in
the southern-most segment of $P_n$ (formally, $A''_n$ is the minimal $y$-coordinate
of a point in $P_n$ and $A'_n$ is the  minimal $x$-coordinate of a point in $P_n$ whose
 $y$-coordinate is $A'_n$). Then $A_n$ should be close to the middle of the south edge $S_n:=(0,-n)$.

We can define likewise $B_n, C_n, D_n$, which should be close respectively to
$E_n,N_n, W_n$ where $E=(n,0)$ etc. See the figure.
Finally, we denote by $X:\R^2\to\R$, resp. $Y$, the projection on the first
(resp. second) coordinate. Then we have


\begin{itemize}
\item
$d(A_n,S_n)/n$ converges in distribution to 0 (and likewise for $d(B_n,E_n)/n$ etc.)
\item
The part of the boundary of $P_n$ between $A_n$ and $B_n$, converges, after
renormalization, to an arc of parabola (and likewise  between $B_n$ and $C_n$ etc.)
\end{itemize}
A formal statement can be found in Barany.

We want to study the second-order asymptotics.
We need the following estimate, which  is a slight improvement of
Bodini et al. and Bureaux-Enriquez. There exist $C, K>0$ such that
for all sequences $(\delta_n), (\delta'_n)$ satisfying $\delta_n=o(n)$,
$\delta'_n=o(n))$,
the number of convex lattice chains from $(0,0)$ to $(n+\delta_n,n+\delta'_n)$,
contained in $[0, n+\delta_n]\times [0, n+\delta'_n]$ and without vertical steps is given by
\begin{equation}\label{chain}
\exp(C(n+\delta_n)^{1/3}(n+\delta'_n)^{1/3}+H(n+\delta_n,n+\delta'_n)+K\log n+o(1))
\end{equation}
Here $H$ is a corrective term and, using the same arguments as in Bureaux, it can be sen
that uniformly over all $s, t\in \R$,
\begin{equation}\label{H}
|H(n+sn^{2/3},n+tn^{2/3})|=o(n^{1/3})
\end{equation}
On the other hand recall that for fixed reals $s,t>0$,
the number of convex lattice chains from $(0,0)$ to $(sn,tn)$,
contained in $[0, sn]\times [0, tn]$ and such that
$(sn,tn)$ is the only point in the chain whose $x$-coordinate
is $sn$ is given by
\begin{equation}\label{chain2}
\exp(C(sn)^{1/3}(nt)^{1/3}+o(n^{1/3})
\end{equation}

\begin{thm}
(i) The quadruple $$n^{-2/3}(Y(A_n- S_n), X(B_n- E_n),Y(C_n- N_n),X(D_n- W'_n))$$
converges in probability to $\delta_{(0,0,0,0)}$.

(ii)
The quadruple $$n^{-2/3}(X(A_n- S_n), Y(B_n- E_n),-X(C_n- N_n)-Y(D_n- W_n))$$
converges in distribution to a gaussian random variable $(A,B,C,D)$ with
density
$$
C_1\exp\left(-\frac{1}{18}[(r-s)^2+(s-t)^2+(t-u)^2+(u-r)^2]-\frac{1}{3}
[r^2+s^2+t^2+u^2]
\right)
$$
for some normalizing constant $C_1>0$.

(iii)
For every $t\in [0,1]$, let $\AA_n(t)$ be the point of the boudary of $P_n$ tangent to
the vector $(t,1-t)$. Let $\overline{\AA}_n(t)=E(A_n(t)|A_n,B_n)$.
Then the process
$f_n:= (n^{-2/3}(\AA_n(t)-\overline{\AA}_n(t)), t\in[0,1])$ converges in
distribution to a 2-dimensional standard Brownian Bridge.
\end{thm}

Note that $\AA_n(0)=\overline{\AA}_n(0)=A_n$ and $\AA_n(1)=\overline{\AA}_n(1)=B_n$.
Instead of the left-most point $A_n$ of the south edge, we could look at the right-most point
$\tilde{A}_n$. First, remark that $Y(\tilde{A}_n)=Y(A_n)$, so the first part of Theorem 6
would be unchanged. Next, using a formula similar to \eqref{chain} for chains without horizontal
steps instead of chains without vertical steps, the same proof as below would lead to the same result
as (ii) but for $\tilde{A}_n, \tilde{B}_n$ etc. In fact, the distance between $A_n$ and
$\tilde{A}_n$ is of order $n^{1/3}$, as can be seen using the same arguments as in Bodini.\\


Proof

(i) We use the same arguments as in Barany.
A convex lattice polygon can be seen as the union of 4 lattice convex chains.
In particular the number of polygons of this kind contained in
$[-n,n]^2$ is at least the number of such polygons
satisfying $A_n=S_n, B_n=E_n$ etc. which, according to \eqref{chain}, has the form
\begin{equation}\label{centre}
  \exp(4Cn^{2/3}+4K\log n+4H(n,n)+o(1))
  \end{equation}

If $c>0$, if we want to count the number of convex lattice polygons
contained in the rectangle $R_n:=[-n,n]\times[-(n-cn^{(1/3)+\delta}),n]$, we can choose the points
$A_n,B_n,C_n,D_n$ and count the lattice chains in-between. Comparing \eqref{chain} and
\eqref{chain2}, we see that this number is maximized when $A_n,B_n,C_n,D_n$
lie near the middle of the segments of $R_n$. For such a choice of $A_n,B_n,C_n,D_n$,
this  number of convex lattice polygons is bounded above by
$$\exp(4Cn^{1/3}(n-(c/2)n^{2/3})^{1/3}+4H(n, n-(c/2)n^{2/3})+4K\log n+o(1))$$
On the other hand, the number of choices of  $(A_n,B_n,C_n,D_n)$ is bounded $(2n)^4$, so that
the number of convex lattice polygons
contained in $R_n$ is bounded by
$$
\exp(4Cn^{2/3}-\frac{2}{3}Ccn^{1/3} + 4H(n, n-(c/2)n^{2/3})+(4K+16)\log n+o(1))$$
Using \eqref{H}, we obtain
\begin{equation}\label{need}
4H(n,n)>>-\frac{2}{3}Ccn^{1/3} + 4H(n, n-(c/2)n^{2/3})
 \end{equation}
which entails that that the probability that a
random, uniform  convex lattice polygon
contained $[-n,n]^2$ lies in $R_n$ tends to 0 as $n\to\infty$.
So for every $\varepsilon$, with probability going to 1, $n^{-2/3}|Y(A_n- S_n)|<\varepsilon$
and we have the same estimates for $B_n, C_n, D_n$.

(ii) From (i), we know that there exists a sequence $(D_n)$ of integers such that $D_n=o(n^{2/3})$
and that with probability going to 1, $|Y(A_n)+n|<D_n$, $|X(B_n)-n|<D_n$ etc.
Let now $(\delta_n,\delta'_n,\delta''_n,\delta'''_n)$ be sequences of integers such that for each $n$,
$0<\delta_n<D_n$ etc. We want to study the law of 
$$n^{-2/3}(X(A_n- S_n), Y(B_n- E_n),-X(C_n- N_n)-Y(D_n- W_n))$$
conditionally on the event
$${\bf E}_n=\{Y(A_n- S_n)=\delta_n, X(B_n- E_n)=\delta'_n,Y(C_n- N_n)=\delta''_n,
X(D_n- W'_n)=\delta'''_n\}$$
Fix $r,s,t,u \in\R$. For simplicity, we shall omit the integer part notation in the sequel.
We want to estimate the number of 4-tuple of convex chains such that
\begin{eqnarray*}
&&X(A_n- S_n)=rn^{2/3}, Y(A_n- S_n)=\delta_n\\
&&Y(B_n- E_n)=sn^{2/3}, X(B_n- E_n)=\delta'_n
\end{eqnarray*}
etc.
Let $L_n(r,s,t,u)$ denote the logarithm of the number of such 4-tuples of
chains. The number of chains going from $A_n$ to $B_n$ is the same as the number of chains
from $(0,0)$ to $(n-\delta'_n-rn^{2/3},n-\delta_n+sn^{2/3})$. According to \eqref{chain}, this leads to
\begin{eqnarray*}
  \L_n(r,s,t,u)&=&Cn^{2/3}\left(\left(1-\frac{r}{3n^{1/3}}-\frac{2r^2}{9n^{2/3}}-\frac{\delta'_n}{n}
                   +O(1/n)\right)
    \left(1+\frac{s}{3n^{1/3}}-\frac{2s^2}{9n^{2/3}}-\frac{\delta_n}{n}+O(1/n))\right)\right)\\
&&+H\left(n-rn^{2/3}-\delta'_n,n+sn^{2/3}-\delta_n \right)+k\log n +\ldots
\end{eqnarray*}
where we only wrote the term corresponding to the chain from $A_n$ to $B_n$ but of course, there are
3 other terms. Summing up, we see that terms of the form $r/n^{1/3}$ cancel out and we get
\begin{eqnarray*}
  L_n(r,s,t,u)&=&Cn^{2/3}\left(4+ 2\left(\frac{\delta_n}{n}+\frac{\delta'_n}{n}+\frac{\delta''_n}{n}
                          +\frac{\delta'''_n}{n}\right)
                      -\frac{4}{9}\left(\frac{r^2+s^2+t^2+u^2}{n^{2/3}}\right)
                         -\frac{1}{9}\left(\frac{rs+st+tu+ur}{n^{2/3}}\right)\right)\\
                      &&+4K \log n+H\left(n-rn^{2/3}-\delta'_n,n+sn^{2/3}-\delta_n \right)+\ldots
                         +O(1/n)
\end{eqnarray*}
where again, in the last line, we have 3 additional terms involving the function $H$.
In particular, we get
$$
\frac{L_n(r,s,t,u)}{Cn^{2/3}}=\frac{L_n(0,0,0,0)}{Cn^{2/3}}
-\frac{1}{18}[(r-s)^2+(s-t)^2+(t-u)^2+(u-r)^2]-\frac{1}{3}
[r^2+s^2+t^2+u^2]+o(1)
$$
using the following fact that follows from \eqref{H}:
\begin{equation}\label{need1}
|H\left(n-rn^{2/3}-\delta'_n,n+sn^{2/3}-\delta_n \right)-
H\left(n-\delta'_n,n-\delta_n \right)|=o(n^{2/3})
\end{equation}
etc.

This is true for all sequences $(\delta_n,\delta'_n,\delta''_n,\delta'''_n)$, which completes the
proof.


(iii) We just use the same proof as in Section 5.

==> historique/1dec_introduction.tex <==

% ==================Intro Zono==================

The study of large convex lattice polytopes, starting with the famous
question of their enumeration asked by Arnold, has been a long standing
question where, in dimension $\geq 3$, all natural problems regarding
their asymptotic shape remain essentially open. 

In this context, the study of lattice zonotopes, a subclass of convex lattice
polytopes whose definition is given below, seems more tractable.
In particular, Barany-Bureaux-Lund proved that in any dimension, in a given cone,
the shape of large  zonotopes converges to a deterministic limit after
rescaling.

Following this result, it is natural to investigate the second order
asymptotics. As one gets a deterministic limit in a first approximation,
it seems reasonable to expect gaussian fluctuations. However, since the
limiting shape is convex and thus is twice differentiable almost everywhere,
it may not be completely obvious that the fluctuations could be gaussian and therefore
related to Brownian motion, which is a much more irregular object, namely
H\"older $1/2-\varepsilon$- continuous.

Nevertheless, we do get gaussian fluctuations in the following sense.
Take a vector $u\in\R^d$ and let $A_u$ be the point of a $d$-dimensional
zonotope tangent to $u$. Then the fluctuations of $A_u$ from its mean are gaussian
with normalising factor $n^{1/(d+1)}$.

To be more precise, recall that a zonotope in $\mathbb{R}^d$ is defined as the
Minkowski sum of a finite set $E$ of vectors $\in \mathbb{R}^d$, the vectors in $E$
being called the generators of the zonotope.
 If we restrict ourselves to vectors with nonnegative
 integer coordinates and such that the $\sum_{v\in E}=(n,n\ldots n)$, we get a finite number of
 zonotopes and if we pick one uniformly at random,  we get the following 


\begin{thm}
  Let $Z_n$ be a random zonotope starting at the origin, ending at $(n,n\ldots n)$, and composed
  of generators in $\N^d$. Let $\uu\in\R^d$ and let $\AA^n_{\uu}$ be the point of $Z_n$ that is
  tangent to the hyperplane with normal vector $\uu$.
  Then there exists a symmetric matrix $\Gamma_\uu$, given in \ref{thm:CLT}, such that
  $$ (n^{-\frac{d+2}{d+1}}\Gamma_{\uu}) ^{-1/2}\left(\AA^n_{\uu} -E(\AA^n_{\uu})\right) \overset{(d)}{\underset{n\rightarrow \infty}{\longrightarrow}} N$$
  where $N$ is a standard, $d$-dimensional gaussian variable.
\end{thm}



We point out that, while the boundary of a $d$-dimensional zonotope is a
$d-1$-dimensional object, the fluctuations of the tangent point
$\AA_u$ are $d$-dimensional fluctuations.

Let us mention that we have an explicit expression, not only for $\Gamma_{\uu}$ but also for
$E(\AA^n_{\uu})$. More generally, we obtain a $k$-point version of the result: if one takes a family
$u_1, \ldots u_k$ of vectors and looks at the tangent points $\AA^n_{u_1}, \ldots \AA_{u_k}$,
then the $k$-tuple $(\AA^n_{u_1}-E(\AA^n_{u_1}), \ldots \AA^n_{u_k}-E(\AA^n_{u_k}))$
converges in law to a gaussian random vector with an explicit covariance structure, see Theorem ?

Finally, the result of convergence in distribution can be refined and we a get local limit theorem.
See Section 3.


In the 2-dimensional case, zonogons are just centrally symmetric
convex lattice polygons. Another way to state this is that a convex
lattice polygon is the union of four arcs of zonogons, each of these arcs being an arc of parabola,
as shown in the seminal papers of Barany, Sinai and Vershik. In this setting, our result on
fluctuations can be extended to a functional limit theorem as in Donsker's theorem. Moreover,
This Donsker-type result on zonogons can be generalized for general polygons contained in a
square.

To be more precise, consider a random, uniform lattice convex polygon $P_n$ contained in the
square $[-n,n]^2$.
Let $A_n=(A'_n, A''_n)$ be the western-most point in
the southern-most segment of $P_n$ and $S_n$ be the ``south pole'', that is, $S_n=(0,-n)$. 
We can define likewise $B_n, C_n, D_n$, which should be close respectively to
$E_n,N_n, W_n$ where $E=(n,0)$ etc. See the figure.
Finally, we denote by $X:\R^2\to\R$, resp. $Y$, the projection on the first
(resp. second) coordinate. 

\begin{figure}[h]
    \centering
    \def\svgscale{1}
    \includesvg[width = 250pt]{images/polygone.svg}
\end{figure}


\begin{thm}
(i) The quadruple $$n^{-2/3}(Y(A_n- S_n), X(B_n- E_n),Y(C_n- N_n),X(D_n- W'_n))$$
converges in probability to $\delta_{(0,0,0,0)}$.

(ii)
The quadruple $$n^{-2/3}(X(A_n- S_n), Y(B_n- E_n),-X(C_n- N_n)-Y(D_n- W_n))$$
converges in distribution to a gaussian random variable $(A,B,C,D)$ with
density
$$
C_1\exp\left(-\frac{1}{18}[(r-s)^2+(s-t)^2+(t-u)^2+(u-r)^2]-\frac{1}{3}
[r^2+s^2+t^2+u^2]
\right)
$$
for some normalizing constant $C_1>0$.

(iii)
For every $t\in [0,1]$, let $\AA_n(t)$ be the point of the boudary of $P_n$ tangent to
the vector $(t,1-t)$. Let $\overline{\AA}_n(t)=E(A_n(t)|A_n,B_n)$.
Then there exists a family of $2\times 2$  matrices $(M(t), 0\leq t\leq 1)$, such that the process
$$(n^{-2/3}M(t)(\AA_n(t)-\overline{\AA}_n(t)), t\in[0,1])$$ converges in
distribution to a 2-dimensional standard Brownian Bridge.
\end{thm}



%===================Plan=======================
The next section connects integral zonotopes and strict integer partitions. Section 3 is about the limiting zonoid and some examples. The basic
probabilistic model and proofs of the main results are in Section 4. Section 5 establishes several combinatorial properties of a typical zonotope T
in T (C, k), namely we estimate the number of i-dimensional faces of T,
for $i = 0, 1, . . . , d - 1$. Section 6 includes proofs of the existence of limit
shapes for integral zonotopes chosen in arbitrary convex bodies in R
2
, and
in hypercubes for higher dimensions.


\leavevmode\\






==> historique/3_old_version.tex <==
Given a zonogone $Z$ with positive generators, let $Z^+$ (resp. $Z-$) be the upper (resp. lower) polygonal line of $Z$. Without loss of generalities, we will study $Z^+$ in the following. Let $\{\AA^n_\uu\}_{\uu \in \R_{-} \times \R_{+} }$ be a stochastic process encoding the point of contact between $Z^{+}$ and the hyperplane normal to $\uu$. The vector $\uu$ is normalised relatively to the 1-norm, therefore $\uu = (u-1, u)$ with $u \in [0,1]$.\\

% esperance toujours valide pour \aa_n ? $\boldsymbol{\mu}_\uu = (u^2, 2u - u^2)$\\

Let$\boldsymbol{\Tilde{\AA}}^n_{\uu}$ be the stochastic process defined as: $$\boldsymbol{\Tilde{\AA}}^u_{\uu} = \frac{1}{n^{2/3}} \left(\AA^n_\uu -  \mathbb{E}\left[ \AA^n_\uu \right] \right)$$

and let $\BB^n_{t}$ be the stochastic process of the tangent point to the normal vector $(t-1, t)$, $t$ being between 0 and 1, for the zonotopes that \textbf{end at $n\kk$}. 

$$ \BB^n_{t} =\boldsymbol{\Tilde{\AA}}^n_{(t-1,t)}. $$


{\color{red} Il faut le meme theorem pour les points $\aa_{n}(s,r) = \left(n+ s n^{\frac{2}{3}}, n+ r n^{\frac{2}{3}} \right) $ difference entre le cone pour $k$ et le cone pour $k_n$. Il faut argument d'encadrement (mais attention a la monotonie)\\
Ou alors garder la proba P_n, mais conditionner au point d'arrivée a_n}

\begin{thm}\label{thm:Donsker}
Let $r$ and $s$ be positive numbers. Suppose $Z_n\in \mathcal{Z}(\mathbb{R}^2, n\boldsymbol{1})$ a random zonogon drawn under $P_n$, composed of positive generators and ending at the point $\aa_{n}(s,r) = \left(n+ s n^{\frac{2}{3}}, n+ r n^{\frac{2}{3}} \right)$, and let $\BB^n = \left\{\BB^n_{t}\right\}_{t\in [0,1]}$ the random process defined above for $Z_n$. Then, there exist a nondegenerate diagonal matrix $D(t)$ and an invertible matrix $R(t)$ such that 
$$\BB^n \Rightarrow D^{-1} R \BB R^{-1} $$ 
where $\left\{\BB\left(t^{\frac{1}{4}}\right)\right\}_{t\in [0,1]}$ is the 2-dimensional standard brownian bridge.  
\end{thm}



\begin{prop}[Weak convergence of finite-dimensional distributions]
With the notation of \ref{thm:Donsker}, the finite-dimensional distributions of $\BB^n$ converge weakly to those of $D^{-1} R \BB R^{-1}$.  
\end{prop}  

\begin{proof}  
For any fixed $t$, the probability of $\BB^n_t$ for being $X$ is 
$$\text{P} (\BB^n_t = X ) = \text{P}_n \left(\BB^n_t = X | \AA_{(0,1)} = (n,n) \right) $$  

And with Bayes' theorem  

$$ \text{P} (\BB^n_t = X) = \frac{\text{P}_n \left(\BB^n_t = X, \BB^n_1 - \BB^n_t = - X \right)}{\text{P}_n \left(\AA_{(0,1)} = n \textbf{1} \right)}  $$

$\BB^n_1 - \BB^n_t$ is independent of  $\BB^n_t$ by construction of the probability measure $\text{P}_n$, and satisfy also a local limit theorem. 

$\BB^n_t$ converges toards a Gaussian variable with mean 0 and the following covariance matrix:
$$  \Sigma_t =\left(\frac{\zeta(2)}{\zeta(3)}\right)^{1/3} \begin{pmatrix}
2 t^3 & 3t^2 - 2 t^3 \\
3t^2 - 2 t^3 & 6t - 6t^2 + 2 t^3
\end{pmatrix} $$

Thanks to the coordinate symmetry, $\BB^n_1 - \BB^n_t$ satisfy a local limit theorem towards a Gaussian variable with mean 0 and covariance matrix:

$$ \widetilde{\Sigma}_t =\left(\frac{\zeta(2)}{\zeta(3)}\right)^{1/3} \begin{pmatrix}
6(1-t) - 6(1-t)^2 + 2 (1-t)^3 & 3(1-t)^2 - 2 (1-t)^3 \\
3(1-t)^2 - 2 (1-t)^3 - 2 t^3 & 2 (1- t)^3 
\end{pmatrix} $$

$$ \underset{X \in \mathbb{R}^2}{\sup} \left[\text{P}\left(\BB^n_t = X \right) - \frac{\frac{e^{- \frac{1}{2} X^T \Sigma_t^{-1}X}}{2 \pi |\Sigma_t|} \frac{e^{-\frac{1}{2} X^T \widetilde{\Sigma}_t^{-1} X }}{2 \pi | \widetilde{\Sigma}_t |}}{\frac{1}{2 \pi \left| \Sigma \right|}} \right] \underset{n\rightarrow +\infty}{\rightarrow} 0 $$

Hence there is a local limit theorem for $\BB^n_t$, and therefore a central limit theorem to $\sigma_t N$ where $N$ is a standard normal vector and $\sigma_t$ is a matrix such that :

$$ \sigma_t^2 = \left(\frac{\zeta(2)}{\zeta(3)}\right)^{1/3}  \begin{pmatrix}
-2 \left((4t^2-2t+1\right)t^3(t-1) & \left( 8t^2 - 8t +3 \right) (t-1)^2 t^2 \\
\left( 8t^2 - 8t +3 \right) (t-1)^2 t^2 & -2\left(4t^2 - 6t +3 \right)(t-1)^3 t
\end{pmatrix}$$

\end{proof}


\begin{prop}[Tightness]
for $ 0 \leq r < s < t \leq 1$, and $\alpha >\frac{1}{2}$, and $\beta > 0$

$$\mathbb{E}\left[ \left|\left|\BB^n_s - \BB^n_r \right|\right|_1^2 \left|\left| \BB^n_t-\BB^n_s \right|\right|_1^2 \right] \leq \left| F(t) - F(r)\right|^{2 \alpha}, $$
with $F$ is a nondecreasing, continuous function on $[0,1]$
\end{prop}

\begin{proof}
Let $0 \leq r \leq s \leq t\leq 1$, and . It is sufficient to prove that there exist a constant $C >0$ such that

$$ \mathbb{E}\left[ \left|\left|\BB^n_s - \BB^n_r \right|\right|_1^2 \left|\left| \BB^n_t-\BB^n_s \right|\right|_1^2  \right] \leq C \left(t^3 - r^3\right)^2  .$$


Since $\{\BB^n_t\}$ is a variable on random zonotope that end at $(n,n)$, the first step is to broaden to random zonotopes drawn under Boltzmann measure. The inequality becomes

$$ \frac{1}{n^{8/3}} \mathbb{E}\left[ \left|\left|\AA^n_s - \AA^n_r - \mathbb{E}\left[\AA^n_s - \AA^n_r \right]  \right|\right|_1^2 \left|\left| \AA^n_t-\AA^n_s - \mathbb{E}\left[\AA^n_t - \AA^n_s \right] \right|\right|_1^2  \:\: \left| Z \in \mathcal{Z} \left(\mathbb{N}^2, (n,n) \right) \right.  \right]\leq C \left(t^3 - r^3\right)^2. $$

Writing each difference as a sum over the generators, one can notice that this expectancy will result in a sum over quadruplets primitive generators $\{ \xx_1, \xx_2 \xx_3, \xx_4 \}$, and the probability for each quadruplet to occur respectively $k_1, k_2, k_3$, and $k_4$ is

$$ \text{P}(k_1, k_2, k_3, k_4) =\prod_{i=1}^4 \text{P}_n \left( \omega(\xx_i) = k_i \right) \frac{\text{P}_n \left(  \AA_1^n \setminus \{\xx_1,\xx_2,\xx_3,\xx_4\} = (n,n) - \sum_{i=1}^4 k_i \xx_i \right)}{\text{P}_n \left( \AA_1^n = (n,n)\right)} $$


Yet the local limit theorem ensures that there exist $n_1$ large enough such that for $n> n_1$, for any $\{ \xx_1, \xx_2 \xx_3, \xx_4 \}$, the ratio is bounded : 

$$ \frac{\text{P}_n \left(  \AA_1^n \setminus \{\xx_1,\xx_2,\xx_3,\xx_4\} = (n,n) - \sum_{i=1}^4 k_i \xx_i \right)}{\text{P}_n \left( \AA_1^n = (n,n)\right)} \leq 2 $$

Therefore, it remains

$$  \mathbb{E}\left[ \left|\left|\BB^n_s - \BB^n_r \right|\right|_1^2 \left|\left| \BB^n_t-\BB^n_s \right|\right|_1^2  \right] \leq \frac{2}{n^{8/3}} \mathbb{E}\left[ \left|\left|\AA^n_s - \AA^n_r - \mathbb{E}\left[\AA^n_s - \AA^n_r \right]  \right|\right|_1^2 \left|\left| \AA^n_t-\AA^n_s - \mathbb{E}\left[\AA^n_t - \AA^n_s \right] \right|\right|_1^2 \right]$$

The remaining expectancy can be split in two parts due to independence. Denoting $\mathcal{C}_{r,s} = \left\{ \xx \in \R, \xx \cdot (r-1, r) \leq 0 \leq \xx \cdot (s-1, s) \right\}$ and $\alpha_{\xx} = \xx \left( \omega(\xx) - \mathbb{E}[\omega(\xx)]\right) = (\alpha_{\xx,1},\alpha_{\xx,2})$ respectively the cone of vectors contributing to $\AA^n_s - \AA^n_r$ and the weight of each vector in the expectancy, it becomes

$$ \frac{2}{n^{4/3}} \mathbb{E}\left[ \left(\sum_{\xx \in \mathbb{P}^2 \cap \mathcal{C}_{r,s} } \alpha_{\xx,1} \right)^2 
+ \left(\sum_{\xx \in \mathbb{P}^2 \cap \mathcal{C}_{r,s} } \alpha_{\xx,2} \right)^2 +
\left|\left(\sum_{\xx \in \mathbb{P}^2 \cap \mathcal{C}_{r,s} } \alpha_{\xx,1} \right)\left(\sum_{\xx \in \mathbb{P}^2 \cap \mathcal{C}_{r,s} } \alpha_{\xx,2} \right)\right| \right]    $$


Those terms are terms of the covariance matrix of $\AA^n_s - \AA^n_r$ that have been calculated previously in this paper using Proposition 1. Corollary 1 gives a upper bound independent of the radius of the cone (i.e. independent of $r-s$):


Therefore for $n_2$ large enough, \\ 
 
$$ \frac{2}{n^{4/3}} \mathbb{E}\left[ \left(\sum_{\xx \in \mathbb{P}^2 \cap \mathcal{C}_{r,s} } \alpha_{\xx,1} \right)^2 
 \right] \leq 8 \left(\frac{\zeta(2)}{\zeta(3)}\right)^{1/3} (s^3 - r^3) $$
 
 Finally, $(s^3 - r^3)(t^3 - s^3) \leq (t^3 - r^3)^2$ concludes the proof.

\end{proof}




$$P_n(\AA_\uu = X | Z \in Z( \mathcal{C}, n \kk) ) = \frac{P_n(\AA_\uu = X) P_n( \AA_{(1,1)} - \AA_\uu = n \kk - X )}{P_n\left( Z \in Z( \mathcal{C}, n \kk) \right)}  $$

Expressing the covariance, using $t= \frac{u_2}{u_1+ u_2}$, hence $t\in [0,1]$:

$$\Sigma_t =\left(\frac{\zeta(2)}{\zeta(3)}\right)^{1/3} n^{4/3} \begin{pmatrix}
2 t^3 & 3t^2 - 2 t^3 \\
3t^2 - 2 t^3 & 6t - 6t^2 +  2 t^3
\end{pmatrix} $$


{\color{blue} Il faut que le resultat soit étendu à des chemins $(n+ s n^{2/3},n+ d n^{2/3}) $ uniformément sur $s$ et $d$. Notamment dans la prop3}






